Aligned Datasets Improve Detection of Latent Diffusion-Generated Images

As latent diffusion models (LDMs) democratize image generation capabilities, there is a growing need to detect fake images. A good detector should focus on the generative models fingerprints while ignoring image properties such as semantic content, resolution, file format, etc. Fake image detectors are usually built in a data driven way, where a model is trained to separate real from fake images. Existing works primarily investigate network architecture choices and training recipes. In this work, we argue that in addition to these algorithmic choices, we also require a well aligned dataset of real/fake images to train a robust detector. For the family of LDMs, we propose a very simple way to achieve this: we reconstruct all the real images using the LDMs autoencoder, without any denoising operation. We then train a model to separate these real images from their reconstructions. The fakes created this way are extremely similar to the real ones in almost every aspect (e.g., size, aspect ratio, semantic content), which forces the model to look for the LDM decoders artifacts. We empirically show that this way of creating aligned real/fake datasets, which also sidesteps the computationally expensive denoising process, helps in building a detector that focuses less on spurious correlations, something that a very popular existing method is susceptible to. Finally, to demonstrate just how effective the alignment in a dataset can be, we build a detector using images that are not natural objects, and present promising results. Overall, our work identifies the subtle but significant issues that arise when training a fake image detector and proposes a simple and inexpensive solution to address these problems.

==> old.tex <==
% To generate an image using a diffusion model, a noise has to be iteratively refined over many denoising steps. Therefore, collecting a big set of such fake images (e.g., 10k-100k) will require a lot of compute and time. So, how do we generate something that is still a product of the same generative model, but faster? Our idea is to \emph{reconstruct the real images}. The reason this can be much quicker is because the popular latent diffusion models (LDMs) in use today \cite{rombach2022highresolutionimagesynthesislatent} have an autoencoder that can be used to compress and decompress an RGB image in a single forward pass. So, even though the reconstruction looks the same as its corresponding real image to the human eye, it still has the artifacts introduced due to the decoder of the autoencoder. And since anything being generated by the LDM, including the aforementioned noise generated images, will have to pass through the same decoder, they will share the same artifacts. We use this principle to train a neural network based classifier on real vs real-reconstructions. We conduct thorough experiments to show how this method performs equally well, and in some cases, better, than the existing baselines.  



% \section{Misaligned Datasets Induce False Pattern Learning}
% Fake image detection focuses on identifying subtle differences. It is important to make sure that the model does not pick up on false patterns. These include artifacts caused by compression, resizing etc. In this section, we analyze ways in which this problem could arise. We categorize them into \textbf{Training-Induced Artifacts} and \textbf{Data Artifacts}. For demonstration purposes, we consider the detector trained by \cite{corvi2022detectionsyntheticimagesgenerated}, which suffers from both kinds of problems.  
% \\\\
% \subsection{TRAINING-INDUCED ARTIFACTS}



% For a fake image detector to be of practical use, we also want it to be robust with respect to common post processing operations such as resizing, compression etc. A common way to achieve this is by performing data augmentation using these operations during training. The desired behaviour is for the augmentations to create similar artifacts on both real and fake images, so that the detector becomes invariant to these artifacts. If this does not occur, the detector could focus on these features resulting in the detector potentially focusing on incorrect patterns. We refer to these kinds of artifacts as Training-Induced Artifacts. The detector trained by \cite{corvi2022detectionsyntheticimagesgenerated} learns to associate downsampling with real images and upsampling with fake images as a result of the training pipeline.
% \\\\
% \textbf{Experimental Details}: We consider a set of real images from the Redcaps \cite{desai2021redcapswebcuratedimagetextdata} dataset, for convenience, we select 200 images of the resolution 512x512. For our fake images, we generate 200 fake images of the resolution 512x512 using prompts that correspond to categories from the CIFAR dataset. We measure and report the average probability of an image being detected as a fake image. We sweep across all resolutions from 128x128 till 1024x1024 with increments of 10.
% \\\\
% \textbf{Analysis}: Fig \ref{fig:1} displays the behaviour of the ResNet-50 trained by \cite{corvi2022detectionsyntheticimagesgenerated} with respect to both upsampling and downsampling. The convolution operation is not equivariant to resizing. Therefore, CNN's are not invariant to resizing. This problem is commonly addressed by either introducing inductive biases in the architecture \cite{sosnovik2020scaleequivariantsteerablenetworks, worrall2019deepscalespacesequivariancescale} or via data augmentation. \cite{corvi2022detectionsyntheticimagesgenerated} use the latter approach. One such augmentation is the RandomResizedCrop augmentation. The RandomResizedCrop takes in a source image and takes a random crop from the image. This random crop is then resized to a target resolution. Their approach resizes the cropped image to a final resolution of 256x256. During training, the model is expected to see images that have been resized in different ways. As a result the learned detector should become more robust towards resizing. The dataset used by \cite{corvi2022detectionsyntheticimagesgenerated} generates all fake images at 256x256. Whereas the real image dataset is a mixture of the COCO and LSUN datasets. The COCO dataset has images of different resolutions, mostly occupying larger areas than a 256x256 image. This results in the corresponding random crops also being larger than the final size, this results in these images being predominantly downsampled. However, since the fake images are already at the final resolution, upsampling is the only operation performed on the crops. Therefore, during training, any artifact of downsampling is associated with a real image which the model learns. At the same time, upsampling artifacts are more often associated with fake images. This is a major issue during inference, since resizing is one of the most common operations. While this issue could potentially be overcome by being more careful with the training pipeline, we argue that a more general solution is obtained through better dataset alignment.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\textwidth]{sweeps/Corvi2023.png} 
%     \caption{Your caption here}
%     \label{fig:1}
% \end{figure}
% \\
% \subsection{DATA-INDUCED ARTIFACTS}
% It is important to make sure that the real and fake images are processed in the same manner. However, given that most of our real images are scraped from the internet, we are not aware of the exact post-processing operation that was applied to every single one of them. This could force the model to focus on incorrect artifacts. We refer to these as Data-Induced Artifacts. We demonstrate that due to the way in which the LSUN \cite{yu2016lsunconstructionlargescaleimage} was processed, the detector learns to associate webp compression artifacts with real images.

% \textbf{Experimental Details}

% \textbf{Analysis}




%\section{Training-Induced False Pattern Learning}
%While training a fake-image detector, it is important to make sure that they are not sensitive to post-processing operations. A common strategy is to make these models invariant to post-processing operations via use of data augmentations. In this section, we demonstrate that using data augmentations can introduce false patterns which can be used for classification. We analyze the fake image detector trained by \cite{corvi2022detectionsyntheticimagesgenerated} where we observe that their model tends to associate downsizing artifacts with real images and up-sampling artifacts with fake images. 

%\textbf{Experimental Details}: We consider a set of real images from the Redcaps \cite{desai2021redcapswebcuratedimagetextdata} dataset, for convenience, we select 200 images of the resolution 512x512. For our fake images, we generate 200 fake images of the resolution 512x512 using prompts that correspond to categories from the CIFAR dataset. We measure and report the average probability of an image being detected as a fake image. We sweep across all resolutions from 128x128 till 1024x1024 with increments of 10.

%\textbf{Analysis}: The convolution operation is not equivariant to resizing. Therefore, CNN's are not invariant to resizing. This problem is commonly addressed by either introducing inductive biases in the architecture \cite{sosnovik2020scaleequivariantsteerablenetworks, worrall2019deepscalespacesequivariancescale} or via data augmentation. \cite{corvi2022detectionsyntheticimagesgenerated} use the latter approach. One such augmentation is the RandomResizedCrop augmentation. The RandomResizedCrop takes in a source image and takes a random crop from the image. This random crop is then resized to a target resolution. Their approach resizes the cropped image to a final resolution of 256x256. Their fake images are generated at the resolution of 256x256, therefore the process of taking a crop and resizing it to 256x256 will always introduce up-sampling artifacts. The real images are taken from the COCO and LSUN datasets. The COCO images are mostly bigger than 256x256 whereas the LSUN images are of the resolution 256x256. Therefore, downsizing artifacts are only associated with the real images forcing the model to associate downsizing with real images. Similarly, since the up-sampling operation is more likely to be associated with a fake image than with a real image. While this issue can be mitigated with more careful design of the pipeline, we argue that a simpler and more general solution can be obtained by simply reconstructing the real images using the generative model.

%\section{Reconstructing the real dataset}
%A useful property of a generative model is the ability to take in a real image and find a latent that can closely reconstruct the given image. This property is present in a lot of generative models such as VAE's, GAN's and diffusion models. The reconstructed real image is also a fake image since it is generated by the same model that we look to defend against. Therefore, we propose to create our fake images by reconstructing all the real images. Our study predominantly focuses on Stable Diffusion, for which we use the corresponding VAE \cite{kingma2022autoencodingvariationalbayes, oord2018neuraldiscreterepresentationlearning} to reconstruct the images. We also demonstrate that the same can be achieved for pixel space diffusion models using DDIM inversion \cite{song2022denoisingdiffusionimplicitmodels}.



%\subsection{Training with Reconstructions Avoids Spurious Correlations}
%We claimed that by ensuring proper training dataset alignment, we can reduce the chance of the detector learning spurious correlations. In this section, we test our hypothesis. We test this out by seeing if our approach can mitigate the issues with resizing which we discussed earlier.\\\\
%\textbf{Experiment Details}: We randomly select 500 real images from the Redcaps \cite{desai2021redcapswebcuratedimagetextdata} dataset. We also generate 500 images using SD-v1.5 (prompts pertain to object categories from the CIFAR \cite{krizhevsky2010cifar} dataset). All the collected images have a resolution of 512x512. We start by downsampling both real and fake images to a base resolution of 128x128 (scaling factor of 0.25). The mean probability value given by the detector is then measured. Then we increment the base resolution by 10 and repeat the same process until we reach 1024x1024 (scaling factor of 2). This way, we test evaluate the model on both upsampling as well as downsampling. We plot the mean probability of the images being fake versus the scaling factor. 


%\textbf{Results and Discussion}: The robustness of our detectors is shown in Fig \ref{fig:rzsweep}. We notice that the baseline detector's performance (blue curve) on fake images Fig \ref{fig:rzsweep}-left falls almost immediately as we start downsizing them. The performance of our method falls at a slower rate, struggling only when faced with extreme downsampling. Similarly, when upsampling real images, the performance of the baseline detector worsens whereas our detector is not as sensitive. This is an encouraging sign, demonstrating that careful alignment of the datasets reduces the likelihood of the model learning spurious correlations.

%\textbf{Training Details}: Following the work of \cite{corvi2022detectionsyntheticimagesgenerated} we finetune a ResNet-50 \cite{he2015deepresiduallearningimage} for fake image detection. We use \emph{ResNet-50 (Baseline)} while referring to a detector that was not trained on reconstructions. While training on the dataset that we designed, we train the model in two ways,
% \begin{itemize}
%     \item \emph{ResNet-50 (Ours)}: In a mini-batch, the images are randomly selected (no alignment in the mini-batch). However, the reconstructions still exist in the overall dataset.
%     \item \emph{ResNet-50 (Ours-sync)}: In a mini-batch, we select a set of real images and their reconstructions. We make sure to apply the exact same augmentation on the real image and its reconstruction in a given batch. 
% \end{itemize}

% \begin{itemize}
%     \item Real: Consists of 1000 natural images taken from Reddit \cite{desai2021redcapswebcuratedimagetextdata}, 1000 artistic-looking real images taken from wikiart and LAION-Aesthetics. We also use 1000 face images taken from whichfaceisreal.com.
%     \item SD: Consists of 3000 fake images generated by the SD family. We use 1000 images each from the InstructPix2Pix \cite{brooks2023instructpix2pixlearningfollowimage} training dataset and Nights \cite{fu2023dreamsimlearningnewdimensions} dataset. Another 1000 images are generated by reconstructing the face images present in our real test dataset using DDIM inversion.
%     \item Midjourney: We take 3000 images generated by Midjourney. Midjourney is a closed-source commercial model. 
%     \item Kandinsky: We take 1000 images generated by the Kandinsky \cite{razzhigaev2023kandinskyimprovedtexttoimagesynthesis} model. The Kandinsky model uses a different VAE and UNet compared to the original LDM model.
%     \item Playground: We use Playground-v2.5 \cite{li2024playgroundv25insightsenhancing} to generate 3000 images. We use 100 captions generated by ChatGPT as our prompts. Playground-v2.5 is architecturally identical to SD-XL \cite{podell2023sdxlimprovinglatentdiffusion}. The UNet is 3-times larger than that of the original LDM, but the VAE has a similar architecture.
%     \item PixelArt-$\alpha$: We use PixelArt-$\alpha$ \cite{chen2023pixartalphafasttrainingdiffusion} to generate 3000 images to a set of ChatGPT generated prompts. The model uses a Diffusion Transformer \cite{peebles2023scalablediffusionmodelstransformers} as the UNet backbone.
% \end{itemize}

%We make sure that our testing images has both natural and artistic looking images. The selected models offer a wide range of architectural choices utilized by latent diffusion models. Furthermore, we also evaluate the robustness of the detectors to common post-processing operations, such as JPEG compression, blurring, color jitter, and others.

% \subsection{Using reconstructions improves robustness}
% In this section we evaluate fake image detectors on the above-mentioned dataset. We conduct experiments in both a lab setting (clean, unprocessed images) and a open-world setting (random JPEG, blur etc),

